$I=1$ $\pi$-$\pi$ scattering at the physical point

We present a preliminary analysis of $I=1$ $\pi\,\pi$ scattering at the physical point. We make use of the stochastic variant of the distillation framework (also known as sLapH) to compute the relevant two-point correlation matrices using a basis of single and multihadron interpolating operators to estimate the low energy spectra. We perform the L\"uscher analysis to determine the scattering phase shift which is finding good agreement with the experimentally obtained phase shifts.

==> I=1 - scattering at the physical point/macro.tex <==

\newcommand\bef{\begin{figure}}
\newcommand\eef[1]{\label{fg:#1}\end{figure}}
\newcommand\bec{\begin{center}}
\newcommand\eec{\end{center}}
\newcommand\besf{\begin{subfigure}}
\newcommand\eesf[1]{\label{sfg:#1}\end{subfigure}}
\newcommand\beq{\begin{equation}}
\newcommand\eeq[1]{\label{#1}\end{equation}}
\newcommand\beqa{\begin{eqnarray}}
\newcommand\eeqa[1]{\label{#1}\end{eqnarray}}
\newcommand\bet{\begin{table}}
\newcommand\eet[1]{\label{tb:#1}\end{table}}
\newcommand\best{\begin{subtable}}
\newcommand\eest[1]{\label{stb:#1}\end{subtable}}
\newcommand\betb{\begin{center}\begin{tabular}}
\newcommand\eetb{\end{tabular}\end{center}}
\newcommand\beit{\begin{itemize}}
\newcommand\eeit{\end{itemize}}

\newcommand\fgn[1]{Figure \ref{fg:#1}}
\newcommand\eqn[1]{eq.\ (\ref{#1})}
\newcommand\scn[1]{Section \ref{s:#1}}
\newcommand\sscn[1]{Section \ref{ss:#1}}
\newcommand\ssscn[1]{Section \ref{sss:#1}}
\newcommand\tbn[1]{Table \ref{tb:#1}}
\newcommand\ttbn[1]{\ref{tb:#1}}
\newcommand\stbn[1]{Table \ref{stb:#1}}
\newcommand\tstbn[1]{\ref{stb:#1}}
\newcommand\apxn[1]{Appendix \ref{s:#1}}
\newcommand{\nn}{\nonumber}
\newcommand{\eps}{\epsilon}
\newcommand{\ot}{\otimes}
\newcommand{\op}{\oplus}
\newcommand{\om}{\ominus}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\threehalf}{\frac{3}{2}}
\newcommand{\fivehalf}{\frac{5}{2}}
\newcommand{\sevenhalf}{\frac{7}{2}}
\newcommand{\ninehalf}{\frac{9}{2}}
\newcommand{\osq}{\frac{1}{\sqrt{2}}}
\newcommand{\ra}{\rangle}
\newcommand{\bref}[1]{{\raggedright \scriptsize #1}}
\newcommand{\lref}[1]{{\hfill       \scriptsize #1}}
\newcommand{\cref}[1]{\bec  \textcolor{black}{\small #1}\eec}
\newcommand{\aref}[1]{\textcolor{gray}{\scriptsize #1}}

\newcommand\dadt[4]{[\bar{#1}\bar{#2}]_{3_c}[#3 #4]_{\bar{3}_c}}
\newcommand\dads[4]{[\bar{#1}\bar{#2}]_{\bar{6}_c}[#3 #4]_{6_c}}
\newcommand\dad[4]{[\bar{#1}\bar{#2}]_{\bar{\mathcal{G}}}[#3 #4]_{\mathcal{G}}}
\newcommand\dq[2]{[#1 #2]}
\newcommand\twomeson[4]{[\bar{#1} #2]_{\mathcal{G}}[\bar{#3} #4]_{\mathcal{G}}} 
\newcommand\twomesonsa[4]{[\bar{#1} #2]_{1_c}[\bar{#3} #4]_{1_c}}
\newcommand\twomesonsb[4]{[\bar{#1} #2]_{1_c}[ #4\bar{#3}]_{1_c}}



\newcommand\incfig[2]{\includegraphics[scale=#1]{plots/#2}}
\newcommand\self[1]{{\color{blue}\bf Note to ourselves: #1}}
\newcommand\pblu[1]{{\color{blue}\bf #1~}}
\newcommand\rblu[1]{{\color{blue}\bf #1}}
\newcommand\prblu[1]{{\color{blue} #1~}}
\newcommand\pbla[1]{{\color{black}\bf #1~}}
\newcommand\mblu[1]{{\mathbin{\color{blue}\bf #1}}}
\newcommand\mred[1]{{\mathbin{\color{red}\bf #1}}}
\newcommand\mgre[1]{{\mathbin{\color{green}\bf #1}}}
\newcommand\pred[1]{{\color{red}\bf #1~}}
\newcommand\pgre[1]{{\color{green}\bf #1~}}

\newcommand\au[2]{#1{(#2)}}
\newcommand\aul[3]{#1^{+#2}_{-#3}}
\newcommand\auls[4]{#1^{+#2}_{-#3}{(\pm#4)}}

\newcommand\AV{{\scriptscriptstyle AV}}
\newcommand\eint{E_{\rm int}}
\newcommand\had{{\scriptscriptstyle H}}
\newcommand\Nm{{\scriptscriptstyle N_-}}
\newcommand\Np{{\scriptscriptstyle N_+}}
\newcommand\PS{{\scriptscriptstyle PS}}
\newcommand\SC{{\scriptscriptstyle S}}
\newcommand\V{{\scriptscriptstyle V}}
\newcommand\x[1]{{\mathbf{#1}}}
\newcommand\mn[1]{\mathnormal{#1}}

\newcommand\cdof{\chi^2/\mathrm{DOF}}
\newcommand\ie{{\sl i.e.\/}}
\newcommand\etc{{\sl etc\/.}}
\newcommand\tr{\mathrm{Tr}\;}
\newcommand\formul{formul{\ae}}
\newcommand\etal{{\sl et al.\/}}

\newcommand\epj{{\sl Eur.\ Phys.\ J.\/}\ }
\newcommand\jhep{{\sl J.\ H.\ E.\ P.\/}\ }
\newcommand\np{{\sl Nucl.\ Phys.\/}\ }
\newcommand\npbps{{\sl Nucl.\ Phys.\/} B ({\sl Proc. \ Suppl.\/})\ }
\newcommand\pos{{\sl PoS\/}\ }
\newcommand\pr{{\sl Phys.\ Rev.\/}\ }
\newcommand\pls{{\sl Phys.\ Lett.\/}\ }
\newcommand\prlt{{\sl Phys.\ Rev.\ Lett.\/}\ }
\newcommand\arxiv[2]{{arXiv:#1 ~[#2]}\ }

\newcommand{\beginbackup}{
   \newcounter{framenumbervorappendix}
   \setcounter{framenumbervorappendix}{\value{framenumber}}
}
\newcommand{\backupend}{
   \addtocounter{framenumbervorappendix}{-\value{framenumber}}
   \addtocounter{framenumber}{\value{framenumbervorappendix}} 
}

\definecolor{DarkGreen}{rgb}{0.00,0.29,0.00}
\definecolor{DarkRedfooter}{rgb}{0.60,0.00,0.00}
\definecolor{DarkRed}{rgb}{0.60,0.00,0.00}
\definecolor{DarkRedtitle}{rgb}{0.85,0.00,0.00}

\newenvironment{changemargin}[3]{%
\begin{list}{}{%
\setlength{\topsep}{#1}%
\setlength{\leftmargin}{#2}%
\setlength{\rightmargin}{#3}%
\setlength{\listparindent}{\parindent}%
\setlength{\itemindent}{\parindent}%
\setlength{\parsep}{\parskip}%
}%
\item[]}{\end{list}}

\def\prsp#1#2%
  {\mathop{}%
   \mathopen{\vphantom{#2}}^{#1}%
   \kern-\scriptspace%
   #2}



